Spatiotemporal Graph Neural Networks in short term load forecasting: Does adding Graph Structure in Consumption Data Improve Predictions?

Short term Load Forecasting (STLF) plays an important role in traditional and modern power systems. Most STLF models predominantly exploit temporal dependencies from historical data to predict future consumption. Nowadays, with the widespread deployment of smart meters, their data can contain spatiotemporal dependencies. In particular, their consumption data is not only correlated to historical values but also to the values of neighboring smart meters. This new characteristic motivates researchers to explore and experiment with new models that can effectively integrate spatiotemporal interrelations to increase forecasting performance. Spatiotemporal Graph Neural Networks (STGNNs) can leverage such interrelations by modeling relationships between smart meters as a graph and using these relationships as additional features to predict future energy consumption. While extensively studied in other spatiotemporal forecasting domains such as traffic, environments, or renewable energy generation, their application to load forecasting remains relatively unexplored, particularly in scenarios where the graph structure is not inherently available. This paper overviews the current literature focusing on STGNNs with application in STLF. Additionally, from a technical perspective, it also benchmarks selected STGNN models for STLF at the residential and aggregate levels. The results indicate that incorporating graph features can improve forecasting accuracy at the residential level; however, this effect is not reflected at the aggregate level

==> legacy/02__background.tex <==
% \subsubsection*{1. Encoding Phase}
% The encoder maps the input sequence \( \{\mathbf{x}_t\}_{t=1}^T \) into a latent representation \( \mathbf{H} \):
% \begin{equation}
%     \mathbf{H} = \text{TEMP}_{\text{enc}}\left(\{\mathbf{x}_t\}_{t=1}^T\right),
% \end{equation}
% where:
% \begin{itemize}
%     \item \( \text{TEMP}_{\text{enc}} \): A generic operator (e.g., RNN, CNN, or MLP) that captures temporal dependencies or patterns in the input sequence.
%     \item \( \mathbf{H} \): Encoded representation, which could be a sequence of hidden states (e.g., from RNNs) or a fixed-dimensional vector (e.g., from CNNs or MLPs).
% \end{itemize}

% \subsubsection*{2. Decoding Phase}
% The decoder generates the forecasted sequence \( \{\mathbf{y}_{t'}\}_{t'=T+1}^{T+H} \) based on the encoded representation \( \mathbf{H} \):
% \begin{equation}
%     \mathbf{y}_{t'} = \text{TEMP}_{\text{dec}}\left(\mathbf{H}, \{\mathbf{y}_{t''}\}_{t''=T+1}^{t'-1}\right), 
% \end{equation}
% where:
% \begin{itemize}
%     \item \( \text{TEMP}_{\text{dec}} \): A generic operator that maps the encoded representation and previous outputs to the current output.
%     \item \( \{\mathbf{y}_{t''}\}_{t''=T+1}^{t'-1} \): Previously predicted outputs, used in an autoregressive manner.
% \end{itemize}

% \subsubsection*{1. Encoder}
% \begin{equation}\label{rec}
%     \mathbf{h}_t = \text{TEMP}\left(\mathbf{x}_t\right)
% \end{equation}

% where:
% \begin{itemize}
%     \item \( \mathbf{x}_t \): Input vector at timestep \( t \).
%     \item \text{TEMP} is an encoder which process data in temporal order.
% \end{itemize}

% \subsubsection*{2. Decoder}
% \begin{equation}
%     \mathbf{y}_t = \mathcal{F}_y\left(\mathbf{h}_t\right)
% \end{equation}

% where:
% \begin{itemize}
%     \item \( \mathbf{y}_t \): Output vector at timestep \( t \).
%     \item \( \mathcal{F}_y \): A generic function that maps the hidden state to the output (e.g \acrshort{mlp}).
% \end{itemize}


% In this paradigm, operations are executed in two steps:

% \subsubsection*{1. Message Aggregation}
% \[
% \mathbf{m}_v^{(l)} = \text{AGGREGATE}^{(l)}\left(\{\mathbf{h}_u^{(l-1)} : u \in \mathcal{N}(v)\}\right)
% \]
% where:
% \begin{itemize}
%     \item \( \mathbf{h}_u^{(l-1)} \): Feature vector of node \( u \) at layer \( l-1 \).
%     \item \( \mathcal{N}(v) \): Set of neighbors of node \( v \).
%     \item \( \text{AGGREGATE}^{(l)} \): Permutation-invariant function (e.g., \textit{sum}, \textit{mean}, \textit{max} or \textit{attention-based mechanism}).
% \end{itemize}

% \subsubsection*{2. Feature Update}
% \[
% \mathbf{h}_v^{(l)} = \text{UPDATE}^{(l)}\left(\mathbf{h}_v^{(l-1)}, \mathbf{m}_v^{(l)}\right)
% \]
% where \( \text{UPDATE}^{(t)} \) is a learnable function (e.g., neural network).
% % \begin{itemize}
% %     \item 
% % \end{itemize}

% \subsubsection*{Output Computation}
% The node abstract representations are mapped to desired outputs.
% \begin{equation}
%     \mathbf{y}_v = \mathcal{F}_y\left(\mathbf{h}_v\right)
% \end{equation}

% This architecture takes the reverse order of equations (\ref{equ:tts}) (3). Specifically, by propagating in the spatial dimension, we obtain spatial respenstation of all population in time stamp. Sequentially, a learnable function, such as a \acrshort{cnn} or \acrshort{mlp}, processes information in temporal dimension. This architecture closely resembles the \acrshort{tas} approach, with the distinction that \acrshort{tas} employs \acrshort{rnn} models to recursively takes spatial representations in each time step.

% Block of \inlinebox{\adjustbox{valign=B}{\colorbox{Blue}{$X_i^{t}$}}} represents load consumption $\mathbf{X} \in \mathbb{R}^{N\times T}$ of N consumers in from period $[t, t+T)$.

    % \begin{subfigure}[b]{0.23\textwidth}
    %     \centering
    %     
    % \end{subfigure}

    % \hfill
    % \begin{subfigure}[b]{0.14\textwidth}
    %     \centering
    %     \includegraphics[width=\linewidth]{assets/stt.pdf}
    %     \caption{\acrshort{stt} architecture}
    %     \label{fig:stt}
    % \end{subfigure}

% \paragraph{STEGNN~\cite{wei_short-term_2023}} This model incorporates a graph formation learning mechanism from~\cite{wu_connecting_2020}. Furthermore, it employs a moving average graph convolutional layer to smooth out the transition between multiple graph layers. At this stage, the model processes only data in the spatial axis. Then a \acrshort{mlp} model capture transformed features for forecasting. This model is therefore of type \acrshort{stt}.

% Table \ref{tab:overview} gives an overview of some \acrshort{stgnn}s in the literature that fit to the framework we introduced in previous sections.
 
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
